The Cosmological OTOC: A New Proposal for Quantifying Auto-Correlated Random Non-Chaotic Primordial Fluctuations

The underlying physical concept of computing out-of-time-ordered correlation (OTOC) is a significant new tool within the framework of quantum field theory, which now-a-days is treated as a measure of random fluctuations. In this paper, by following the canonical quantization technique, we demonstrate a computational method to quantify the two different types of cosmological auto-correlated OTO functions during the epoch when the non-equilibrium features dominates in primordial cosmology. In this formulation, two distinct dynamical time scales are involved to define the quantum mechanical operators arising from the cosmological perturbation scenario. We have provided detailed explanation regarding the necessity of this new formalism to quantify any random events generated from quantum fluctuations in primordial cosmology. We have performed an elaborative computation for the two types of two-point and four-point auto-correlated OTO functions in terms of the cosmological perturbation field variables and its canonically conjugate momenta to quantify random auto-correlations in the non-equilibrium regime. For both of the cases, we found significantly distinguishable non-chaotic, but random, behaviour in the OTO auto-correlations, which was not pointed out before in this type of study. Finally, we have also demonstrated the classical limiting behaviour of the mentioned two types of auto-correlated OTOC functions from the thermally weighted phase-space averaged Poisson brackets, which we found to exactly match the large time limiting behaviour of the auto-correlations in the super-horizon regime of the cosmological scalar mode fluctuation.

==> Makefile <==
# makefile
#
# 2019 Nov 01
#
# Macro definitions
#
# - parameters:
ROOT_NAME	= halloweenmath
#   (the following need not be redefined, although it can be)
BUNDLE_NAME	= $(ROOT_NAME) package
#
# - all the rest:
DTX_NAME	= $(ROOT_NAME).dtx
INS_NAME	= $(ROOT_NAME).ins
LOG_FILE	= $(ROOT_NAME).log
DOC_AUX_FIL	= $(LOG_FILE) $(ROOT_NAME).aux \
				$(ROOT_NAME).glo $(ROOT_NAME).gls \
				$(ROOT_NAME).idx $(ROOT_NAME).ind \
				$(ROOT_NAME).ilg $(ROOT_NAME).glg \
				$(ROOT_NAME).toc $(ROOT_NAME).lof \
				$(ROOT_NAME).hd  $(ROOT_NAME).out
DOCUM_FILE	= $(ROOT_NAME).pdf
CODE_FILES	= $(ROOT_NAME).sty
#
LATEX		= pdflatex
MAKEINDEX	= makeindex
REMOVE		= -rm

#
define GEN_FAKE_INDEX
	@echo '\\begin{theindex}' > $(ROOT_NAME).ind
	@echo '\\end{theindex}'  >> $(ROOT_NAME).ind
	@echo "Generating fake .ind file."
endef
#
define GEN_FAKE_GLOSSARY
	@echo '\\begin{theglossary}' > $(ROOT_NAME).gls
	@echo '\\end{theglossary}'  >> $(ROOT_NAME).gls
	@echo "Generating fake .gls file."
endef



.PHONY: default
.PHONY: code doc
.PHONY: clean cleandoc cleanaux cleancode cleanlog cleanall
.PHONY: help

# Default target
default: doc code

# Generating the code
################################################################
#                                                              #
#   PLEASE NOTE THAT THE INSTALLER SCRIPT IS EXECUTED WITH     #
#       openout_any=r                                          #
#                                                              #
################################################################
code:
	openout_any=r tex $(INS_NAME)

# Generating the documentation
doc: $(DOCUM_FILE)

$(DOCUM_FILE): $(DTX_NAME)
# Hack for getting index and glossary in the toc since first run:
	$(GEN_FAKE_INDEX)
	$(GEN_FAKE_GLOSSARY)
# We know how many runs are needed:
	$(LATEX) $(DTX_NAME)
	$(LATEX) $(DTX_NAME)
	$(MAKEINDEX) -s gind.ist -t $(ROOT_NAME).ilg -o $(ROOT_NAME).ind \
			$(ROOT_NAME).idx
	$(MAKEINDEX) -s gglo.ist -t $(ROOT_NAME).glg -o $(ROOT_NAME).gls \
			$(ROOT_NAME).glo
	$(LATEX) $(DTX_NAME)
	$(LATEX) $(DTX_NAME)
# Hyperlinks in the indexes seem not to work properly without the
# following additional run:
	$(MAKEINDEX) -s gind.ist -t $(ROOT_NAME).ilg -o $(ROOT_NAME).ind \
			$(ROOT_NAME).idx
	$(MAKEINDEX) -s gglo.ist -t $(ROOT_NAME).glg -o $(ROOT_NAME).gls \
			$(ROOT_NAME).glo
	$(LATEX) $(DTX_NAME)

# Cleaning up: command "make clean" defaults to "make cleanall"
clean: cleanall

# Cleaning the code files
cleancode:
	$(REMOVE) $(CODE_FILES)

# Cleaning the documentation files
cleandoc: cleanaux
	$(REMOVE) $(DOCUM_FILE)

# Cleaning just the auxiliary files used in producing the documentation
cleanaux:
	$(REMOVE) $(DOC_AUX_FIL)

# Cleaning only the transcript file (e.g., after "make code")
cleanlog:
	$(REMOVE) $(LOG_FILE)

# Cleaning up all the generated files
cleanall: cleancode cleandoc

# Giving help
help:
	@echo "Here is a list of the available commands:"
	@echo
	@echo "  make"
	@echo "    Generate both the code and the documentation (see below)."
	@echo
	@echo "  make code"
	@echo "    Generate all the LaTeX \"executables\" (e.g., \`.sty' files)"
	@echo "    of the $(BUNDLE_NAME);"
	@echo "    these files go into the LaTeX input directories."
	@echo
	@echo "  make doc"
	@echo "    Generate the documentation (in PDF); the resulting PDF file"
	@echo "    goes into the LaTeX documentation directories (the auxiliary"
	@echo "    files may be discarded)."
	@echo
	@echo "  make clean"
	@echo "  make cleanall"
	@echo "    These two commands are synonyms; they remove all of the"
	@echo "    generated files (both code and documentation)."
	@echo
	@echo "  make cleancode"
	@echo "    Remove the LaTeX source files (the \"code files\")."
	@echo
	@echo "  make cleandoc"
	@echo "    Remove the documentation, together with all the auxiliary"
	@echo "    files used to generate it."
	@echo
	@echo "  make cleanaux"
	@echo "    Remove only the auxiliary files used to generate the"
	@echo "    documentation."
	@echo
	@echo "  make cleanlog"
	@echo "    Remove just the transcript file (e.g., after \"make doc\")."
	@echo
	@echo "  make help"
	@echo "    Print this help message."
	@echo



==> OTOC2 2/Makefile <==
# makefile
#
# 2019 Nov 01
#
# Macro definitions
#
# - parameters:
ROOT_NAME	= halloweenmath
#   (the following need not be redefined, although it can be)
BUNDLE_NAME	= $(ROOT_NAME) package
#
# - all the rest:
DTX_NAME	= $(ROOT_NAME).dtx
INS_NAME	= $(ROOT_NAME).ins
LOG_FILE	= $(ROOT_NAME).log
DOC_AUX_FIL	= $(LOG_FILE) $(ROOT_NAME).aux \
				$(ROOT_NAME).glo $(ROOT_NAME).gls \
				$(ROOT_NAME).idx $(ROOT_NAME).ind \
				$(ROOT_NAME).ilg $(ROOT_NAME).glg \
				$(ROOT_NAME).toc $(ROOT_NAME).lof \
				$(ROOT_NAME).hd  $(ROOT_NAME).out
DOCUM_FILE	= $(ROOT_NAME).pdf
CODE_FILES	= $(ROOT_NAME).sty
#
LATEX		= pdflatex
MAKEINDEX	= makeindex
REMOVE		= -rm

#
define GEN_FAKE_INDEX
	@echo '\\begin{theindex}' > $(ROOT_NAME).ind
	@echo '\\end{theindex}'  >> $(ROOT_NAME).ind
	@echo "Generating fake .ind file."
endef
#
define GEN_FAKE_GLOSSARY
	@echo '\\begin{theglossary}' > $(ROOT_NAME).gls
	@echo '\\end{theglossary}'  >> $(ROOT_NAME).gls
	@echo "Generating fake .gls file."
endef



.PHONY: default
.PHONY: code doc
.PHONY: clean cleandoc cleanaux cleancode cleanlog cleanall
.PHONY: help

# Default target
default: doc code

# Generating the code
################################################################
#                                                              #
#   PLEASE NOTE THAT THE INSTALLER SCRIPT IS EXECUTED WITH     #
#       openout_any=r                                          #
#                                                              #
################################################################
code:
	openout_any=r tex $(INS_NAME)

# Generating the documentation
doc: $(DOCUM_FILE)

$(DOCUM_FILE): $(DTX_NAME)
# Hack for getting index and glossary in the toc since first run:
	$(GEN_FAKE_INDEX)
	$(GEN_FAKE_GLOSSARY)
# We know how many runs are needed:
	$(LATEX) $(DTX_NAME)
	$(LATEX) $(DTX_NAME)
	$(MAKEINDEX) -s gind.ist -t $(ROOT_NAME).ilg -o $(ROOT_NAME).ind \
			$(ROOT_NAME).idx
	$(MAKEINDEX) -s gglo.ist -t $(ROOT_NAME).glg -o $(ROOT_NAME).gls \
			$(ROOT_NAME).glo
	$(LATEX) $(DTX_NAME)
	$(LATEX) $(DTX_NAME)
# Hyperlinks in the indexes seem not to work properly without the
# following additional run:
	$(MAKEINDEX) -s gind.ist -t $(ROOT_NAME).ilg -o $(ROOT_NAME).ind \
			$(ROOT_NAME).idx
	$(MAKEINDEX) -s gglo.ist -t $(ROOT_NAME).glg -o $(ROOT_NAME).gls \
			$(ROOT_NAME).glo
	$(LATEX) $(DTX_NAME)

# Cleaning up: command "make clean" defaults to "make cleanall"
clean: cleanall

# Cleaning the code files
cleancode:
	$(REMOVE) $(CODE_FILES)

# Cleaning the documentation files
cleandoc: cleanaux
	$(REMOVE) $(DOCUM_FILE)

# Cleaning just the auxiliary files used in producing the documentation
cleanaux:
	$(REMOVE) $(DOC_AUX_FIL)

# Cleaning only the transcript file (e.g., after "make code")
cleanlog:
	$(REMOVE) $(LOG_FILE)

# Cleaning up all the generated files
cleanall: cleancode cleandoc

# Giving help
help:
	@echo "Here is a list of the available commands:"
	@echo
	@echo "  make"
	@echo "    Generate both the code and the documentation (see below)."
	@echo
	@echo "  make code"
	@echo "    Generate all the LaTeX \"executables\" (e.g., \`.sty' files)"
	@echo "    of the $(BUNDLE_NAME);"
	@echo "    these files go into the LaTeX input directories."
	@echo
	@echo "  make doc"
	@echo "    Generate the documentation (in PDF); the resulting PDF file"
	@echo "    goes into the LaTeX documentation directories (the auxiliary"
	@echo "    files may be discarded)."
	@echo
	@echo "  make clean"
	@echo "  make cleanall"
	@echo "    These two commands are synonyms; they remove all of the"
	@echo "    generated files (both code and documentation)."
	@echo
	@echo "  make cleancode"
	@echo "    Remove the LaTeX source files (the \"code files\")."
	@echo
	@echo "  make cleandoc"
	@echo "    Remove the documentation, together with all the auxiliary"
	@echo "    files used to generate it."
	@echo
	@echo "  make cleanaux"
	@echo "    Remove only the auxiliary files used to generate the"
	@echo "    documentation."
	@echo
	@echo "  make cleanlog"
	@echo "    Remove just the transcript file (e.g., after \"make doc\")."
	@echo
	@echo "  make help"
	@echo "    Print this help message."
	@echo


